Seesaw: High-throughput LLM Inference via Model Re-sharding

To improve the efficiency of distributed large language model (LLM) inference, various parallelization strategies, such as tensor and pipeline parallelism, have been proposed. However, the distinct computational characteristics inherent in the two stages of LLM inference-prefilling and decoding-render a single static parallelization strategy insufficient for the effective optimization of both stages. In this work, we present Seesaw, an LLM inference engine optimized for throughput-oriented tasks. The key idea behind Seesaw is dynamic model re-sharding, a technique that facilitates the dynamic reconfiguration of parallelization strategies across stages, thereby maximizing throughput at both phases. To mitigate re-sharding overhead and optimize computational efficiency, we employ tiered KV cache buffering and transition-minimizing scheduling. These approaches work synergistically to reduce the overhead caused by frequent stage transitions while ensuring maximum batching efficiency. Our evaluation demonstrates that Seesaw achieves a throughput increase of up to 1.78x (1.36x on average) compared to vLLM, the most widely used state-of-the-art LLM inference engine.

==> content/algo/schedule.tex <==
\begin{algorithm}[tb]
   \caption{Scheduling}
   \label{alg:schedule}
\begin{algorithmic}
    \STATE {\bfseries Input:} prompt set $inputs$
    \STATE {\bfseries Output:} 
    \STATE $waiting \gets inputs$, $prefilled \gets \varnothing$
    \STATE $prefetched \gets \varnothing$, $decoding \gets \varnothing$
    \REPEAT
    \IF {$status = prefill$}
        \IF {CPU KV is full}
            \STATE switch to decode
        \ELSE
            \STATE return schedule prefill
        \ENDIF
    \ELSE
        \IF {CPU KV is empty}
            \STATE switch to prefill
        \ENDIF
        \IF {GPU KV is not full}
            \STATE $decode\_batch \gets sample \in $ 
        \ENDIF
    \ENDIF
    \UNTIL{$waiting=\varnothing$}
\end{algorithmic}
\end{algorithm}

==> content/drafts/intro_0.tex <==
\section{Introduction}

% Background: why LLMs are important?
Large language models (LLMs), such as the LLaMA~\cite{llama} and GPT~\cite{gpt4} series, have recently demonstrated significant efficacy across a wide range of applications, including chatbots~\cite{chatgpt}, code assistants~\cite{copilot}, databases management~\cite{llm-sql}, and knowledge graphs processing~\cite{graphrag}, etc. 
% briefly introduce LLM generation process, which is used afterwards.
These models operate by generating output tokens in response to input prompts, a process that can be divided into two distinct stages: \emph{prefill}, which involves the initial processing of the input, and \emph{decode}, which produces the corresponding output tokens.

% Parallelzation is an important optimizations. 
% It's necessary for serving large LLMs,
% It can also accelerate; introduce different parallelisms; different parallelism affects performance; has different trade-offs;
To mitigate the huge size and computational demands of LLMs, parallelizaiton, which distributes the inference computation across multiple devices, is a critical optimization~\cite{demystifying-dist, megatron}.
It enables running large-scale models exceeding the memory constraint of a single GPU, and provides acceleration through increased computational resources.
Several parallelization techniques exist, including data parallelism~\cite{preble}, tensor parallelism~\cite{megatron}, and pipeline parallelism~\cite{gpipe,pipedream}, 
each offering different trade-offs in many factors such as inter-connection overhead and memory footprint. 
These parallelization methods can be employed individually or in combination to optimize performance.


% The necessity to pick the optimal strategy.
% It depends on the specific workload.
Selecting the optimal parallelization strategy based on specific workloads is essential for maximizing inference performance~\cite{alpa}.
Different workloads benefit from different parallelization approaches, depending on factors such as memory access patterns, computational intensity, and network communication volume.
For instance, pipeline parallelism introduces lower communication overhead compared to tensor parallelism; however, it diminishes the batching effect by splitting each batch into smaller micro-batches, which increases the frequency of loading weight matrices. As a result, pipeline parallelism is suboptimal in scenarios where maintaining the batching effect is crucial, such as during the decoding stage.

% many studies have shown prefill and decoding are different; We observe show prefill and decoding prefer different parallelisms; Fig
The two stages of LLM-based text generation, namely prefill and decode, exhibit significantly different characteristics~\cite{llmviewer, distserve}.
Prefilling is predominantly compute-bound, whereas decoding is more constrained by memory bandwidth, resulting in distinct trade-offs across parallelization strategies.
As demonstrated in Figure~\ref{}\qd{motivating example}, the optimal configuration for one stage may not be optimal for the other.
Consequently, using a single parallelization strategy for the entire generation process can lead to suboptimal performance in individual stages, causing substantial underutilization of hardware resources.



% We propose a performance model
To gain deeper insight into this phenomenon, we propose a performance model to analyze optimal deployment strategies across various scenarios, based on detailed profiling data. This model accounts for multiple factors influencing performance, including parallelism, memory bandwidth and capacity, computational resources, interconnection networks, and workload characteristics. It offers an intuitive yet effective framework for evaluating performance in LLM inference, enabling more informed decisions about parallelization strategies. 
% Explain perf model in details
We decompose the runtime of each forward pass of the LLM into data movement, computation, and inter-connection overheads,
and consider how each parallelism affects these components.
The main insights given by the performance model include:
1) Only tensor parallelism can effectively accelerate the data movement of weight matrices, which is substantial in decoding;
2) The all-reduce overhead does not scale with the degree of tensor parallel. On contrary, its absolute runtime even increases while other components are accelerated, making it quickly become the largest overhead, especially in prefilling. On the other hand, pipeline and data parallelism effectively eliminates the all-reduce overhead;
3) While data and pipeline parallelism manifests similar property regarding data movement and all-reduce overhead, they also have different trade-offs. Data parallelism suffer from larger memory occupation by the duplicated weights, which leads to smaller maximum batch sizes. On the other hand, pipeline parallelism can hardly achieve its performance upper bound due to constraints including bubbles and peer-to-peer communication.


Based on the observation and analysis, we propose a new technique called \emph{model re-sharding}. 
It allows selecting different parallelism strategies respectively for prefilling and decoding, and dynamically switch between them during runtime.
The transition is achieved by re-distributing the model weights as well as the KV-cache.
In contrast, existing LLM inference frameworks typically rely on a single parallelization strategy, resulting in suboptimal performance.~\qd{we need to workaround for DistServe} 
Model re-sharding is particularly effective for offline, large-batch inference tasks that prioritize throughput.
Applications that benefit from this technique include database processing~\cite{llm-sql}, knowledge graph processing~\cite{graphrag}, benchmarking~\cite{narayan2022can}. 
% High-throughput offline inference is a class of applications, database, rag, knowledgegraph...

% Re-sharding is contradictory with continuous batching.
However, dynamically switching between different parallelisms conflicts with with continuous batching~\cite{orca}, which batches generation requests in the granularity of tokens and admits new requests as existing requests complete, in order to maximize the number of concurrent requests. To overcome this challenge, we propose a CPU memory offloading technique, where we pre-compute the KV-cache of a large batch of requests, which is then offloaded to CPU memory, and loading it back  continuously to fill empty GPU memory. By carefully coordinating the overlap between data movement and computation, we effectively hide the overhead of swapping between CPU and GPU memory.

We implement \sys{} as a high-throughput oriented LLM inference engine. The evaluation shows \sys{} achieves XX\% average speedup and up to YY\% improvement of throughput compared with the state-of-the-art LLM inference engine.

To summarize, our main contributions include
\begin{itemize}
\item Identify the problem of different preference of parallelisms in the prefilling and decoding, especially for throughput-oriented applications;
\item Build a performance model to analyze the tradeoffs of different parallelization strategies;
\item Propose \emph{model re-sharding}, which allows selecting different parallelization strategies for prefilling and decoding;
\item Conduct a comprehensive evaluation of \sys{} with realistic workloads.
\end{itemize}

% Based on the performance model and experimental observations, we specifically optimize for two cases, namely 1) in-GPU throughput-oriented, and 2) CPU-GPU offloading throughput-oriented. First, in the in-GPU throughput-oriented case, we observe that prefilling and decoding prefer different parallel strategies. We design a \emph{repartition} mechanism that converts the model and KV cache between different configurations. It helps the system achieve optimal throughput in both phases. With model repartition, the throughput of our system is YY\% higher than vLLM.

% Second, for the offloading scenario, we investigate how offloading and parallelism work in synergy. The configuration given by our performance model is XX\% faster than the state-of-the-art offloading system FlexGen.

% TODO: 

==> content/drafts/intro_1.tex <==
Recent advances in large language models (LLMs), exemplified by the Llama~\cite{llama} and GPT~\cite{gpt4} series, have showcased exceptional performance across various domains, including conversational agents~\cite{chatgpt}, automated code generation~\cite{copilot}, database querying~\cite{llm-sql}, and knowledge graph processing~\cite{graphrag}. Alongside these new capabilities, LLM inference introduces significant challenges. Primarily, the substantial computational and memory requirements of LLMs incur considerable operational costs, with inference expenses reportedly reaching billions of dollars. Moreover, studies have demonstrated that scaling model size and computational resources consistently leads to improved LLM performance, driving a trend towards developing increasingly large models (e.g., Llama 3.1 405B). Thus, improving LLM inference efficiency is paramount not only for reducing costs but also enabling the broader scalability of LLM-based applications.

% large size -> necessity of parallelization -> different parallelisms -> need to pick the optimal strategy
As the size of LLMs frequently exceeds the memory capacity of individual GPUs, parallelization is often necessary for deploying these models~\cite{demystifying-dist, megatron}. 
Several parallelization strategies have been proposed, including data, tensor, and pipeline parallelism, which can be applied individually or in combination.
Prior research has demonstrated that each of these strategies presents distinct trade-offs in factors such as memory footprints, inter-device communication overhead, and overall computational efficiency.
The selection of parallelization strategies can significantly impact LLM deployment performance.
For example, a study has shown that applying the optimal configuration for one trace to another can result in up to 2× difference in cost-efficiency.
In our experiments, … (maybe show the maximum performance difference across different parallel configs for the same model deployment)
These findings underscore the importance of selecting appropriate parallelization strategies (in a workload-aware manner) to maximize inference performance.

% statement: static strategy is suboptimal,
% why: two stages have different characteristics
% -> (?) prefer different parallelisms
% -> (?) any fixed strategy might be optimal for the whole process, but suboptimal in each separate stage.

% -> why different characteristics lead to different optimal parallelism (we can skip this point at first)
% -> experiment evidence

Existing research has primarily focused on static parallelization strategies for LLMs, which, once determined, remain fixed throughout execution.
However, our observations reveal that this fixed approach can be suboptimal for LLMs due to their distinct two-stage execution pattern.
The execution of an LLM request comprises two phases: the prefill stage, which processes the initial input sequence of tokens, and the decode stage, which generates tokens one at a time.
As noted in previous studies, these two stages exhibit markedly different computational characteristics.
Prefill is primarily compute-bound, while decoding is often bottlenecked by memory bandwidth.
These differences can result in different optimal parallelization strategies for individual stages.
To illustrate this phenomenon, we measured the individual throughput of the two stages under various parallelization strategies.
Figure X shows ...
Therefore, employing a single parallelization strategy across the entire generation process may lead to suboptimal performance.



==> content/drafts/intro_2.0.tex <==
\section{Introduction}

Emerging large language models (LLMs), such as the Llama~\cite{llama} and GPT~\cite{gpt4} series, have demonstrated exceptional performance across a wide range of tasks. In addition to their widespread use in interactive applications like chatbots~\cite{chatgpt}, LLMs are increasingly utilized in non-interactive, throughput-driven workloads such as information extraction~\cite{narayan2022can}, database querying~\cite{llm-sql}, and knowledge graph processing~\cite{graphrag}. These applications demand substantial computational resources, with a primary focus on maximizing end-to-end throughput. As the scale of models continues to grow (e.g., Llama 3.1~\cite{llama} with 405 billion parameters), the associated computational costs for such tasks have surged considerably. In this work, we focus on improving inference efficiency for throughput-oriented LLM workloads.

As the memory footprints of LLMs frequently exceed the capacity of individual GPUs, parallelization becomes necessary for their deployment ~\cite{demystifying-dist, megatron}. Several parallelization strategies have been proposed, including data, tensor, and pipeline parallelism, which can be used individually or in combination. Prior research highlights that each of these strategies presents distinct trade-offs in factors such as memory footprints, inter-device communication overhead, and computational efficiency. The choice of parallelization strategy can significantly impact LLM inference performance. For instance, using the same hardware, a configuration optimal for one workload may lead to up to $2\times$ lower cost-efficiency when applied to a different workload~\cite{vidur}. These performance discrepancies arise from variations in workload characteristics such as memory access patterns, computational intensity, and network communication volume (more details in Section X). Therefore, adopting workload-aware parallelization strategies is crucial to maximize LLM inference performance.

The execution of an LLM request consists of two phases: the prefill stage, where the initial input sequence of tokens is processed, and the decode stage, where tokens are generated sequentially, one at a time. While numerous studies have proposed methods to optimize parallelization strategies for LLMs, our findings indicate that \emph{a single, static configuration is insufficient to maximize performance across both stages}. As highlighted in prior research, the computational characteristics of these stages differ significantly. The prefill stage is predominantly compute-bound, whereas the decode stage is often constrained by memory bandwidth. These differences suggest that the optimal parallelization strategies for each stage may vary. To illustrate this, we measured the throughput of each stage using different parallelization approaches. (Figure X ...). Hence, relying on a uniform parallelization strategy throughout the generation process can result in suboptimal performance.

\input{content/figs/motivation}

% perf model: runtime = memory (TP's pros) + compute (==) + communication (TP's cons)

% compute same
% communication: TP worst;
% memory: PP - bad batching; DP - duplicate model;

% TP: best at reducing memory access, communication unfriendly;
% PP & DP: memory unfriendly, communication friendly;

% Prefill: %communication larger; leaning towards PP & DP;
% Decode: %memory larger; leaning towards TP;

% Prefill PP++
% Decode TP++;

To elucidate the results presented in Figure X, we analyze how parallelization strategies affect LLM inference performance by breaking down its execution time into three key components: computation, memory access, and communication. Our analysis reveals that while both tensor and pipeline parallelism accelerate computation, they entail significant trade-offs in memory and communication efficiency. Pipeline parallelism, for example, is inefficient in terms of memory access because it requires loading weights multiple times. To enable pipelining, batches are split into micro-batches, which leads to repeated forward passes and the need to load the weights multiple times, resulting in significant memory access overhead. In contrast, tensor parallelism incurs high communication overhead due to the all-reduce operations required at each layer, with execution time increasing as the number of tokens grows. As a result, pipeline parallelism tends to perform better in the prefill stage, where minimizing communication overhead is crucial given the concurrent processing of many tokens. Conversely, tensor parallelism proves more advantageous during the decode stage, where high batching is critical for optimizing performance due to the memory-bound nature of the computations. These findings further underscore the performance limitations of employing a uniform parallelization strategy across both stages.

To address these challenges and optimize performance across both stages, we present \emph{\sys{}}, a high-throughput LLM inference engine that enables adaptive reconfiguration of parallelization strategies between the prefill and decode stages. This adaptability is powered by a novel technique called \emph{dynamic model re-sharding}, which reorganizes model weights and the KV cache during stage transitions to match the memory layout required by the new configuration. This method enables \sys{} to apply parallelization strategies that are specifically tailored to the computational demands of each stage, reducing communication overhead during the prefill stage while enhancing memory efficiency in the decode stage. As a result, \sys{} achieves a significant improvement in overall throughput.


While the concept of model re-sharding appears straightforward, its practical implementation introduces significant challenges. To maximize throughput, existing systems typically adopt prefill-prioritized scheduling, which interleaves prefill and decode stages across batches to achieve continuous batching. However, as illustrated in Figure~\ref{fig:schedule}(a)\qd{TODO: label subfigures}, integrating this approach with dynamic model re-sharding can result in significant overhead due to frequent stage transitions. On the other hand, decode-prioritized scheduling completes all decode steps for a batch before proceeding to the next. While this approach introduces less re-sharding overhead, it suffers from its inherent resource underutilization due to diminishing batching efficiency, as shown in Figure~\ref{fig:schedule}(b). Although other scheduling policies may seek a balance between these two extremes, they remain fundamentally constrained by the trade-off between minimizing re-sharding overhead and mitigating resource underutilization.

\input{content/figs/schedule}

To overcome this constraint and achieve both minimal re-sharding overhead and high batching efficiency, we propose \emph{tiered KV cache buffering}. This method leverages CPU memory as an auxiliary storage unit for the KV cache, enabling \sys{} to precompute and store KV cache data for a substantially larger number of prefill requests. When the CPU cache tier reaches full capacity, \sys{} switches to the decode stage, leveraging the precomputed KV cache to perform decode operations. Once the CPU-stored KV cache is depleted, the system transitions back to the prefill stage. As depicted in Figure~\ref{fig:schedule}(c), this approach ensures that the decoding stage consistently operates with maximal batching efficiency while significantly reducing the frequency of stage transitions, thereby minimizing re-sharding overhead. Notably, transferring KV cache data between CPU and GPU can introduce additional overhead; however, we effectively mitigate this by overlapping data transfers with computation through asynchronous pipelining.

We implement \sys{} as a high-throughput oriented LLM inference engine based on vLLM's model implementation. The evaluation shows \sys{} achieves XX\% average speedup and up to YY\% improvement of throughput compared with the state-of-the-art LLM inference engine.

In summary, we make the following contributions.

\begin{itemize}
\item Identify the problem of different preference of parallelisms in the prefilling and decoding, and analyze the reason behind it;
% \item Build a performance model to analyze the tradeoffs of different parallelization strategies;
\item Propose \emph{dynamic model re-sharding}, allowing reconfiguration of parallelization strategies between the two stages and optimizations tailored to each stage, which improves the throughput;
% \item Propose \emph{tiered KV cache buffering} and \emph{transition-minimized scheduling}, reducing 
\item Conduct a comprehensive evaluation of \sys{} with realistic workloads.
\end{itemize}

==> content/drafts/intro_2.1.tex <==
\section{Introduction}\label{sec:intro}

Emerging large language models (LLMs), such as the Llama~\cite{llama} and GPT~\cite{gpt4} series, have demonstrated exceptional performance across a wide range of tasks. Beyond their prevalent use in interactive applications like chatbots~\cite{chatgpt}, LLLMs are also gaining traction in in non-interactive, throughput-driven workloads such as information extraction~\cite{narayan2022can}, database querying~\cite{llm-sql}, and knowledge graph processing~\cite{graphrag}. 
\qd{Explain some examples in details.}
These workloads prioritize high throughput over low-latency responses, providing opportunities to trade off latency for higher throughput and reduced computational costs.
In this work, we focus on improving inference efficiency for throughput-oriented LLM workloads.

As LLMs often exceed the memory capacity of individual GPUs, parallelization is essential for their deployment ~\cite{demystifying-dist, megatron}. Several parallelization strategies, including \emph{data}, \emph{tensor}, and \emph{pipeline} parallelism, have been proposed, each offering distinct trade-offs in memory, inter-device communication, and computational efficiency. For example, data parallelism~\cite{preble} facilitates parallel computation by replicating the model across devices, but this comes at the expense of significantly increased memory usage.
In contrast, tensor parallelism~\cite{megatron} distributes model weights and computations across devices, which reduces memory overhead but incurs substantial communication costs, as all-reduce operations are performed at each layer.
Pipeline parallelism~\cite{pipedream, gpipe} reduces communication overhead by splitting the model into stages; however, it requires partitioning batches into micro-batches to enable pipelining, which results in multiple forward passes for each batch (see Section~\ref{sec:parallel} for details). Given these trade-offs, the choice of parallelization strategy is generally workload-specific and depends on the unique characteristics of the tasks being executed.

\input{content/figs/motivation}

While numerous studies have proposed methods to optimize parallelization strategies for LLMs~\cite{vllm, alpaserve, scale-transformer}, they typically rely on a single, static configuration throughout the entire generation process.
However, our findings indicate that this fixed approach is often suboptimal due to LLMs' distinct two-phase execution pattern.
The processing of an LLM request consists of two stages: the \emph{prefill} stage, where the initial input sequence of tokens is processed at once to produce the first output token, and the \emph{decode} stage, where tokens are generated one at a time, based on the input and previously generated tokens. As noted in prior studies, the computational characteristics of these stages differ significantly. The prefill stage is primarily compute-bound, handling concurrent processing of multiple tokens from the input prompt. Whereas the decode stage is typically memory-bound, as each step processes only one token at a time for each sequence. These differences suggest that the optimal parallelization strategies for each stage may vary.

To illustrate the performance limitations of applying a uniform parallelization strategy, we measure the execution time of each stage under various combinations of tensor and pipeline parallelism, as shown in Figure~\ref{fig:motivation-example}. We break down the total execution time into three components: weight loading, computation, and communication, to assess their individual contributions to the overall runtime. (1) During the prefill stage, tensor parallelism performs significantly worse than pipeline parallelism due to its high communication overhead. This is because the execution time for all-reduce operations increases proportionally with the large number of tokens processed concurrently in the prefill stage.
(2) In the decode stage, pipeline parallelism is slower than tensor parallelism due to higher weight loading overhead, caused by the increased number of forward passes required for pipelining. This issue is particularly detrimental in the decode stage, where the computation is memory-bound.
Thus, the unique computational characteristics of the prefill and decode stages require different parallelization strategies for optimal performance.
% These findings underscore the performance limitations of employing a uniform parallelization strategy across both stages.

Prior works, such as DistServe~\cite{distserve} and MoonCake~\cite{mooncake}, have explored spatially disaggregating prefilling and decoding. However, these approaches are designed to optimize service-level objectives (SLOs) for online serving rather than maximizing hardware utilization for higher throughput in offline inference. Additionally, they are intended for large clusters with high-speed interconnections, which are not always available. Without such infrastructure, they face limitations due to a restricted search space and bottlenecks caused by slow KV cache transfers. %For example, DistServe does not support GPU systems without peer-to-peer connection.

To address these challenges and optimize performance across both stages, we present \emph{\sys{}}, a high-throughput LLM inference engine that enables adaptive reconfiguration of parallelization strategies between the prefill and decode stages. This adaptability is powered by a novel technique called \emph{dynamic model re-sharding}, which reorganizes model weights and the KV cache during stage transitions to match the memory layout required by the new configuration. This method enables \sys{} to apply parallelization strategies that are specifically tailored to the computational demands of each stage, reducing communication overhead during the prefill stage while enhancing memory efficiency in the decode stage. As a result, \sys{} achieves a significant improvement in overall throughput.


While the concept of model re-sharding appears straightforward, its practical implementation introduces significant challenges. To maximize throughput, existing systems typically adopt prefill-prioritized scheduling~\cite{orca,vllm}, which interleaves prefill and decode stages across batches to achieve continuous batching. However, as illustrated in Figure~\ref{fig:schedule}(a), integrating this approach with dynamic model re-sharding can result in significant overhead due to frequent stage transitions. On the other hand, decode-prioritized scheduling~\cite{faster-transformer} completes all decode steps for a batch before proceeding to the next. While this approach introduces less re-sharding overhead, it suffers from its inherent resource underutilization due to diminishing batching efficiency, as shown in Figure~\ref{fig:schedule}(b). Although other scheduling policies may seek a balance between these two extremes, they remain fundamentally constrained by the trade-off between minimizing re-sharding overhead and mitigating resource underutilization.


To overcome this constraint and achieve both minimal re-sharding overhead and high batching efficiency, we propose \emph{tiered KV cache buffering}. This method leverages CPU memory as an auxiliary storage unit for the KV cache, enabling \sys{} to precompute and store KV cache data for a substantially larger number of prefill requests. When the CPU cache tier reaches full capacity, \sys{} switches to the decode stage, leveraging the precomputed KV cache to perform decode operations. Once the CPU-stored KV cache is depleted, the system transitions back to the prefill stage. As depicted in Figure~\ref{fig:schedule}(c), this approach ensures that the decoding stage consistently operates with maximal batching efficiency while significantly reducing the frequency of stage transitions, thereby minimizing re-sharding overhead. Notably, transferring KV cache data between CPU and GPU can introduce additional overhead; however, we effectively mitigate this by overlapping data transfers with computation through asynchronous pipelining.

\input{content/figs/schedule}
We implement \sys{} as a high-throughput oriented LLM inference engine based on vLLM's model implementation. The evaluation shows \sys{} achieves XX\% average speedup and up to YY\% improvement of throughput compared with the state-of-the-art LLM inference engine.

In summary, we make the following contributions.

\begin{itemize}
\item Identify the problem of different preference of parallelisms in the prefilling and decoding, and analyze the reason behind it;
% \item Build a performance model to analyze the tradeoffs of different parallelization strategies;
\item Propose \emph{dynamic model re-sharding}, allowing reconfiguration of parallelization strategies between the two stages and optimizations tailored to each stage, which improves the throughput;
\item Propose \emph{tiered KV cache buffering}, reducing the model re-sharding overhead;
\item Conduct a comprehensive evaluation of \sys{} with realistic workloads.
\end{itemize}

==> content/drafts/intro_2.2.tex <==
\section{Introduction}\label{sec:intro}

Emerging large language models (LLMs), such as the Llama~\cite{llama} and GPT~\cite{gpt4} series, have demonstrated exceptional performance across a wide range of tasks. Beyond their prevalent use in interactive applications like chatbots~\cite{chatgpt}, LLLMs are also gaining traction in in non-interactive, throughput-driven workloads such as information extraction~\cite{narayan2022can}, database querying~\cite{llm-sql}, and knowledge graph processing~\cite{graphrag}. 
\qd{Explain some examples in details.}
These workloads prioritize high throughput over low-latency responses, providing opportunities to trade off latency for higher throughput and reduced computational costs.
In this work, we focus on improving inference efficiency for throughput-oriented LLM workloads.

As LLMs often exceed the memory capacity of individual GPUs, parallelization is essential for their deployment ~\cite{demystifying-dist, megatron}. Several parallelization strategies, such as \emph{tensor} and \emph{pipeline} parallelism, have been proposed, each offering distinct trade-offs in memory, inter-device communication, and computational efficiency.
% Data parallelism~\cite{preble} processes requests in parallel at the expense of significantly increased memory usage due to replicated models across devices.
Tensor parallelism~\cite{megatron} distributes model weights and computations across devices but incurs substantial communication costs due to all-reduce operations.
In contrary, pipeline parallelism~\cite{pipedream, gpipe} splits the model into stages, has less communication overhead but requires partitioning batches into micro-batches to enable pipelining, which causes repetitive wieght loading (see Section~\ref{sec:parallel} for details).
Given these trade-offs, the choice of parallelization strategy is generally workload-specific and depends on the unique characteristics of the tasks being executed.

\input{content/figs/motivation}

While numerous studies have proposed methods to optimize parallelization strategies for LLMs~\cite{vllm, alpaserve, scale-transformer}, they typically rely on a single, static configuration throughout the entire generation process.
However, our findings indicate that this fixed approach is often suboptimal due to LLMs' distinct two-phase execution pattern.
The processing of an LLM request consists of two stages: the \emph{prefill} stage, where the initial input sequence of tokens is processed at once to produce the first output token, and the \emph{decode} stage, where tokens are generated one at a time, based on the input and previously generated tokens. 
% qidong: too long
As noted in prior studies, the computational characteristics of these stages differ significantly~\cite{llmviewer}.
The prefill stage is primarily compute-bound, handling concurrent processing of multiple tokens from the input prompt. 
Whereas the decode stage is typically memory-bound, as each step processes only one token at a time for each sequence. 
These differences suggest that the optimal parallelization strategies for each stage may vary.

To illustrate the performance limitations of applying a uniform parallelization strategy, we measure the execution time of each stage under various combinations of tensor and pipeline parallelism, as shown in Figure~\ref{fig:motivation-example}. We break down the total execution time into three components: weight loading, computation, and communication, to assess their individual contributions to the overall runtime.
(1) During the prefill stage, tensor parallelism performs significantly worse than pipeline parallelism due to its high communication overhead. 
% This statement is incorrect
This is because the execution time for all-reduce operations increases proportionally with the large number of tokens processed concurrently in the prefill stage.

(2) In the decode stage, pipeline parallelism is slower than tensor parallelism due to higher weight loading overhead, caused by the increased number of forward passes required for pipelining. The weight loading overhead is particularly detrimental in the decode stage, where the computation is memory-bound.
Thus, the unique computational characteristics of the prefill and decode stages require different parallelization strategies for optimal performance.

Prior works, such as DistServe~\cite{distserve} and MoonCake~\cite{mooncake}, have explored spatially disaggregating prefilling and decoding. However, these approaches are designed to optimize service-level objectives (SLOs) for online serving rather than maximizing hardware utilization for higher throughput in offline inference. Additionally, they are intended for large clusters with high-speed interconnections, which are not always available. Without such infrastructure, they face limitations due to a restricted search space and bottlenecks caused by slow KV cache transfers.

To address these challenges and optimize performance across both stages, we present \emph{\sys{}}, a high-throughput LLM inference engine that enables adaptive reconfiguration of parallelization strategies between the prefill and decode stages. This adaptability is powered by a novel technique called \emph{dynamic model re-sharding}, which reorganizes model weights and the KV cache during stage transitions to match the memory layout required by the new configuration. This method enables \sys{} to apply parallelization strategies that are specifically tailored to the computational demands of each stage, reducing communication overhead during the prefill stage while enhancing memory efficiency in the decode stage. As a result, \sys{} achieves a significant improvement in overall throughput.


While the concept of model re-sharding appears straightforward, its practical implementation introduces significant challenges. To maximize throughput, existing systems typically adopt prefill-prioritized scheduling~\cite{orca,vllm}, which interleaves prefill and decode stages across batches to achieve continuous batching. However, as illustrated in Figure~\ref{fig:schedule}(a), integrating this approach with dynamic model re-sharding can result in significant overhead due to frequent stage transitions. On the other hand, decode-prioritized scheduling~\cite{faster-transformer} completes all decode steps for a batch before proceeding to the next. While this approach introduces less re-sharding overhead, it suffers from its inherent resource underutilization due to diminishing batching efficiency, as shown in Figure~\ref{fig:schedule}(b). Although other scheduling policies may seek a balance between these two extremes, they remain fundamentally constrained by the trade-off between minimizing re-sharding overhead and mitigating resource underutilization.

To overcome this constraint and achieve both minimal re-sharding overhead and high batching efficiency, we propose two synergistic techniques \emph{tiered KV cache buffering} and \emph{Transition-minimizing scheduling}. 
Tiered KV cache buffering leverages CPU memory as an auxiliary storage unit for the KV cache, enabling \sys{} to precompute and store KV cache data for a substantially larger number of prefill requests.
Furthermore, \sys{} introduces transition-minimizing scheduling: when the CPU cache tier reaches full capacity, \sys{} switches to the decode stage, leveraging the precomputed KV cache to perform decode operations. Once the CPU-stored KV cache is depleted, the system transitions back to the prefill stage. As depicted in Figure~\ref{fig:schedule}(c), this approach ensures that the decoding stage consistently operates with maximal batching efficiency while significantly reducing the frequency of stage transitions, thereby minimizing re-sharding overhead. Notably, transferring KV cache data between CPU and GPU can introduce additional overhead; however, we effectively mitigate this by overlapping data transfers with computation through asynchronous pipelining.

\input{content/figs/schedule}
We implement \sys{} as a high-throughput oriented LLM inference engine based on vLLM's model implementation. The evaluation shows \sys{} achieves XX\% average speedup and up to YY\% improvement of throughput compared with the state-of-the-art LLM inference engine.

In summary, we make the following contributions.

\begin{itemize}
\item Identify the problem of different preference of parallelisms in the prefilling and decoding, and analyze the reason behind it;
% \item Build a performance model to analyze the tradeoffs of different parallelization strategies;
\item Propose \emph{dynamic model re-sharding}, allowing reconfiguration of parallelization strategies between the two stages and optimizations tailored to each stage, which improves the throughput;
\item Propose \emph{tiered KV cache buffering}, reducing the model re-sharding overhead;
\item Conduct a comprehensive evaluation of \sys{} with realistic workloads.
\end{itemize}

==> content/figs/e2e-l4-a10-all.tex <==
\begin{figure}
    \centering
    \subfigure[Llama3-15B, arxiv]{
    \includegraphics[width=0.47\linewidth, trim={0.4cm, 0.2cm, 0.4cm, 0.2cm}]{figures/e2e-tput/result-a10/llama3-15b_arxiv.pdf}
    }
    \subfigure[CodeLlama-34B, arxiv]{
    \includegraphics[width=0.47\linewidth, trim={0.4cm, 0.2cm, 0.4cm, 0.2cm}]{figures/e2e-tput/result-a10/codellama_arxiv.pdf}
    }\\
    \subfigure[Llama2-70B, arxiv]{
    \includegraphics[width=0.47\linewidth, trim={0.4cm, 0.2cm, 0.4cm, 0.2cm}]{figures/e2e-tput/result-a10/llama70b_arxiv.pdf}
    } 
    \subfigure[Llama3-15B, ShareGPT]{
    \includegraphics[width=0.47\linewidth, trim={0.4cm, 0.2cm, 0.4cm, 0.2cm}]{figures/e2e-tput/result-a10/llama3-15b_sharegpt.pdf}
    }\\
    \subfigure[CodeLlama-34B, ShareGPT]{
    \includegraphics[width=0.47\linewidth, trim={0.4cm, 0.2cm, 0.4cm, 0.2cm}]{figures/e2e-tput/result-a10/codellama_sharegpt.pdf}
    }
    \subfigure[Llama2-70B, ShareGPT]{
    \includegraphics[width=0.47\linewidth, trim={0.4cm, 0.2cm, 0.4cm, 0.2cm}]{figures/e2e-tput/result-a10/llama70b_sharegpt.pdf}
    } 
    \caption{End-to-end Throughput on A10}
    \label{fig:e2e-tput}
\end{figure}

\begin{figure}
    \centering
    \subfigure[Llama3-15B, arxiv]{
    \includegraphics[width=0.47\linewidth, trim={0.4cm, 0.2cm, 0.4cm, 0.2cm}]{figures/e2e-tput/result-aws-l4/llama3-15b_arxiv.pdf}
    }
    \subfigure[CodeLlama-34B, arxiv]{
    \includegraphics[width=0.47\linewidth, trim={0.4cm, 0.2cm, 0.4cm, 0.2cm}]{figures/e2e-tput/result-aws-l4/codellama_arxiv.pdf}
    } \\
    \subfigure[Llama2-70B, arxiv]{
    \includegraphics[width=0.47\linewidth, trim={0.4cm, 0.2cm, 0.4cm, 0.2cm}]{figures/e2e-tput/result-aws-l4/llama70b_arxiv.pdf}
    } 
    \subfigure[Llama3-15B, ShareGPT]{
    \includegraphics[width=0.47\linewidth, trim={0.4cm, 0.2cm, 0.4cm, 0.2cm}]{figures/e2e-tput/result-aws-l4/llama3-15b_sharegpt.pdf}
    } \\
    \subfigure[CodeLlama-34B, ShareGPT]{
    \includegraphics[width=0.47\linewidth, trim={0.4cm, 0.2cm, 0.4cm, 0.2cm}]{figures/e2e-tput/result-aws-l4/codellama_sharegpt.pdf}
    }
    \subfigure[Llama2-70B, ShareGPT]{
    \includegraphics[width=0.47\linewidth, trim={0.4cm, 0.2cm, 0.4cm, 0.2cm}]{figures/e2e-tput/result-aws-l4/llama70b_sharegpt.pdf}
    } 
    \caption{End-to-end Throughput on L4}
    \label{fig:e2e-tput}
\end{figure}

==> content/figs/model.tex <==
\begin{figure*}[t]
    \centering
    \subfloat[L4, 15B, input length = 1k]{
        \includegraphics[width=0.47\linewidth]{figures/l4/llama3-15b.pdf}
    }\hfill
    \subfloat[L4, 34B, input length = 1k]{
        \includegraphics[width=0.47\linewidth]{figures/l4/codellama34b.pdf}
    }\\
    \subfloat[L4, 15B, input length = 4k]{
        \includegraphics[width=0.47\linewidth]{figures/l4-4000/llama3-15b.pdf}
    }\hfill
    \subfloat[L4, 34B, input length = 4k]{
        \includegraphics[width=0.47\linewidth]{figures/l4-4000/codellama34b.pdf}
    }\\
    \subfloat[A10, 15B, input length = 1k]{
        \includegraphics[width=0.47\linewidth]{figures/a10/llama3-15b.pdf}
    }\hfill
    \subfloat[A10, 34B, input length = 1k]{
        \includegraphics[width=0.47\linewidth]{figures/a10/codellama34b.pdf}
    }
    \caption{Comparison between the measured decoding throughput and the predicted value given by our analytical model under different input lengths, GPU models, LLMs and parallelisms. The measured throughput is the obtained by projecting the measured runtime for a single-layer, and the actual batch size can be much smaller than shown in the figure. We use HBM efficiency coefficient 0.8, FLOPS efficiency coefficient 0.5 for L4 and 0.6 for A10.}
    \label{fig:model}
\end{figure*}

==> content/tables/prefill_decode_config.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{c|c|c|c|c|c}
\toprule
& D2T2 & D2P2 & T4 & T2P2 & P4\\
\midrule
\makecell{Prefill Throughput \\ (sequence/s)} & 2.05 & 2.56 & 1.17 & 1.92 & \textbf{2.66} \\
\midrule
\makecell{Decode Throughput \\ (token/s)} & 351 & 235 & \textbf{575} & 495 & 375\\
\bottomrule
\end{tabular}
\caption{Prefilling and decoding prefers different parallelization strategies. Llama13B, L4, prompt\_len=1000}
\label{tab:parallel-config}
\end{table}

==> figures/decode-throughput.tex <==
% \captionsetup{font=footnotesize}
\begin{figure}[th!]\captionsetup[subfigure]{font=small}
    \centering
    % \subfigure[L4, Llama2-13B, len=1k]{
    %     \centering
    %     \includegraphics[width=0.47\linewidth]{figures/par-batch/l4/llama2-13b.pdf}
    % }
    % \hfill
    % \subfigure[L4, Llama3-15B]{
    %     \centering
    %     \includegraphics[width=0.32\linewidth]{figures/par-batch/l4/llama3-15b.pdf}
    % }\hfill
    \subfloat[prompt length=1000]{
        \centering
        \includegraphics[width=0.47\linewidth, trim={0.3cm, 0, 0.3cm, 0}]{figures/par-batch/l4/codellama34b.pdf}
    }\hfill
    % \subfigure[A10, Llama2-13B, len=1k]{
    %     \centering
    %     \includegraphics[width=0.47\linewidth]{figures/par-batch/a10/llama2-13b.pdf}
    % }
    % % \hfill
    % % \subfigure[A10, Llama3-15B]{
    % %     \centering
    % %     \includegraphics[width=0.32\linewidth]{figures/par-batch/a10/llama3-15b.pdf}
    % % }\hfill
    % \subfigure[A10, Llama-34B, len=1k]{
    %     \centering
    %     \includegraphics[width=0.47\linewidth]{figures/par-batch/a10/codellama34b.pdf}
    % }\\
    % \subfigure[L4, Llama2-13B, len=4k]{
    %     \centering
    %     \includegraphics[width=0.47\linewidth]{figures/par-batch/l4-4000/llama2-13b.pdf}
    % }
    % \hfill
    % \subfigure[L4, Llama3-15B, prompt\_len=4k]{
    %     \centering
    %     \includegraphics[width=0.32\linewidth]{figures/par-batch/l4-4000/llama3-15b.pdf}
    % }\hfill
    \subfloat[prompt length=4000]{
        \centering
        \includegraphics[width=0.47\linewidth, trim={0.3cm, 0, 0.3cm, 0}]{figures/par-batch/l4-4000/codellama34b.pdf}
    }
    \caption{Decoding throughput in different scenarios. The optimal parallelism strategy depends on both hardware specifications and workloads. Some observations can be drawn such as 1) TP is efficient with smaller batch sizes, but degenerates with growing batch sizes; 2) The degeneration of TP depends on the ratio between GPU performance and network bandwidth; 3) As the batch size is bounded by the GPU memory and cannot scale infinitely, TP can achieve higher throughput in many cases.}
    \label{fig:parallel-decode}
\end{figure}

==> tables/related-work.tex <==
\begin{table*}[h]
    \centering
    \small
    \begin{tabular}{l | c c |  l  l  c | c  c |  c }
    \toprule
                & Throughput & Latency & TP & PP & re-distribute & \makecell{MLP \\ Offload} & \makecell{Attn \\ Offload}  & Auto Tune \\
    \midrule
      FlexGen~\cite{flexgen}   & \fullcirc{} & \emptycirc{} & \emptycirc{} & \fullcirc{} & \emptycirc{} & \halfcirc{} & \fullcirc{} & \fullcirc{} \\
      HeteGen~\cite{hetegen} & \emptycirc{} & \fullcirc{} & \halfcirc{}\footnotemark[1] & \emptycirc{} & \emptycirc{} & \fullcirc{} & \emptycirc{} & \fullcirc{}\\
      FastDecode~\cite{fastdecode} & \fullcirc{} & \fullcirc{} & \halfcirc{} & \halfcirc{}\footnotemark[1] & \emptycirc{} & \emptycirc{} & \fullcirc{} & \halfcirc{}\\
      InfiniteLLM~\cite{infinite-llm} & \fullcirc{} & \fullcirc{} & \fullcirc{} & \fullcirc{} & \fullcirc{} & \emptycirc{} & \halfcirc{} & \emptycirc{} \\
      Fiddler ~\cite{fiddler} & \emptycirc{} & \fullcirc{} & \emptycirc{} & \emptycirc{} & \emptycirc{} & \fullcirc{} & \emptycirc{} & \fullcirc{}\\
      % MoE-Infinity\footnotemark[2] \\
      LM-Offload~\cite{lm-offload} & \emptycirc{} & \fullcirc{} & \emptycirc{} & \fullcirc{} & \emptycirc{} & \fullcirc{} & \fullcirc{} & \fullcirc{}\\
      % LLM in a flash \\
      Helix~\cite{helix} & \fullcirc{} & \fullcirc{} & \fullcirc{} & \fullcirc{} &\emptycirc{} & \emptycirc{} & \emptycirc{} & \fullcirc{}\\
      SpotServe~\cite{spotserve} &  \fullcirc{} & \fullcirc{} & \fullcirc{} & \fullcirc{} & \fullcirc{} & \emptycirc{} & \emptycirc{} & \fullcirc{}\\
      % MemServe & \\
      Petals~\cite{petals} & \fullcirc{} & \emptycirc{} & \emptycirc{} & \fullcirc{} & \emptycirc{} & \emptycirc{} & \emptycirc{} & \emptycirc{}\\
    % \midrule
      % ours & \fullcirc{} & \fullcirc{} & \fullcirc{} & \fullcirc{} & \fullcirc{} & \fullcirc{} & \fullcirc{} & \fullcirc{}\\
    \bottomrule
      
    \end{tabular}
    \caption{Related Works}
    \label{tab:related-work}
\end{table*}\footnotetext[1]{Between CPU and GPU}
